Calomplification -- The Power of Generative Calorimeter Models

Motivated by the high computational costs of classical simulations, machine-learned generative models can be extremely useful in particle physics and elsewhere. They become especially attractive when surrogate models can efficiently learn the underlying distribution, such that a generated sample outperforms a training sample of limited size. This kind of GANplification has been observed for simple Gaussian models. We show the same effect for a physics simulation, specifically photon showers in an electromagnetic calorimeter.

==> settings.tex <==
% ========================================================================================
% SciPost LaTeX Template (version 2021-08)
% [https://scipost.org/SciPostPhys/authoring#manuprep]
% [https://git.scipost.org/scipost/SciPost_LaTeX_Templates_Submission]
% slightly adapted/customized by Lorenz Vogel (version 2022-01)
% Plehn Group, Institute for Theoretical Physics, Heidelberg University
% [compiler: pdfLaTeX]
% ========================================================================================

\usepackage{jinstpub}

\usepackage[utf8]{inputenc} % input encodings (allow UTF-8 input)
\usepackage[T1]{fontenc} 	% selecting font encodings (use 8-bit T1 fonts)
\usepackage[english]{babel} % multilingual support (English language/hyphenation)

% note: in case the sans serif URL links look jagged/pixelated,
% this may be because you are using MiKTeX and have not yet installed "cm-super"
% solution: first, try to install the "cm-super" package via the "MiKTeX Console"
% alternative: if that doesn't work, the "lmodern" package can be used instead
%\usepackage{lmodern} 		% Latin Modern fonts

% SciPost font typeface and (sans serif or roman) URL style
\usepackage[bitstream-charter]{mathdesign}
\urlstyle{rm} %\urlstyle{sf}

\usepackage{geometry} 		% flexible and complete interface to document dimensions
%\usepackage{microtype} 	% subliminal refinements towards typographical perfection
\usepackage{amsmath} 		% math package (American Mathematical Society)
%\usepackage{amssymb} 		% math package (extended symbol collection)
\usepackage{amsthm} 		% math package (typesetting theorems using AMS style)
\usepackage{mathtools} 		% math package (fixes various deficiencies of amsmath)
\usepackage{float} 			% floating objects such as figures and tables
\usepackage{graphicx} 		% enhanced support for graphics
\usepackage{tabularx} 		% tabulars with adjustable-width columns
\usepackage{booktabs} 		% professional-quality tables
\usepackage{color, xcolor} 	% foreground and background colour management
\usepackage{pdfpages} 		% inclusion of external multi-page PDF documents
\usepackage{extarrows} 		% extra arrows beyond those provided in amsmath
\usepackage{multirow} 		% create tabular cells spanning multiple rows
\usepackage{multicol} 		% intermix single and multiple columns
\usepackage{caption} 		% customising captions in floating environments
\usepackage{subcaption} 	% support for sub-captions (captions for subfigures)
\usepackage{enumitem} 		% control layout of itemize, enumerate, description
\usepackage{setspace} 		% set space between lines (single, onehalf, double)
\usepackage{xspace} 		% define commands that appear not to eat spaces
\usepackage{ragged2e} 		% alternative versions of ragged-type commands
\usepackage{stackrel} 		% enhancement to the \stackrel command
\usepackage{tikz} 			% create PostScript and PDF graphics
\usepackage{braket} 		% Dirac bra-ket notation
\usepackage{bm} 			% access bold symbols in maths mode
\usepackage{tensor} 		% typeset tensors (tensor-style super- and subscripts)
\usepackage{slashed} 		% slash through characters (Feynman slash notation)
\usepackage{siunitx} 		% SI units package (typesetting values with units)
\usepackage{lastpage} 		% reference last page
\usepackage{cite} 			% improved citation handling
\usepackage[normalem]{ulem} % package for underlining
\usepackage{fontawesome} 	% access to web-related icons
\usepackage{tocloft} 		% control over the typography of the TOC, LOF, and LOT
\usepackage{titlesec} 		% interface to sectioning commands (various title styles)
\usepackage{doi} 			% create correct hyperlinks for DOI numbers
\usepackage{hyperref} 		% hypertext links (handel cross-referencing commands)
\usepackage[most]{tcolorbox} 					% coloured and framed text boxes
\usepackage[nameinlink, capitalize]{cleveref} 	% intelligent cross-referencing
\usepackage[nottoc, notlot, notlof]{tocbibind} 	% add references/index/contents to TOC
\usepackage[ruled, vlined]{algorithm2e} 		% floating algorithm environment
%\usepackage{dsfont}             % additional math fonts



% prevent all line breaks in inline equations
\binoppenalty=10000
\relpenalty=10000

\hypersetup{
	pdftitle={Calomplification - The Power of Generative Calorimeter Models},
	pdfauthor={Bieringer et al.},
	colorlinks=true, 			% false: boxed links, true: colored links
	linkcolor={red!50!black}, 	% color of internal links (sections, pages, etc.)
	citecolor={blue!50!black}, 	% color of citation links (links to bibliography)
	urlcolor={blue!80!black} 	% color of URL links (external links)
} 
% more hypersetup options: 
% linktoc=none,section,page,all (defines which part in the TOC is made into a hyperlink)
% hidelinks (removing color and border)

% fix \cal and \mathcal characters look (so it's not the same as \mathscr)
\DeclareSymbolFont{usualmathcal}{OMS}{cmsy}{m}{n}
\DeclareSymbolFontAlphabet{\mathcal}{usualmathcal}




% default setup and general settings
%\sisetup{separate-uncertainty=true}
%\numberwithin{equation}{section}
%\numberwithin{figure}{section}
%\numberwithin{table}{section}

% algorithm environment settings
\renewcommand{\algorithmautorefname}{Algorithm}
\newcommand\mycommfont[1]{\textcolor{gray}{#1}}
\SetArgSty{textnormal}
\SetKwComment{Comment}{{\small\#}~}{}
\SetCommentSty{mycommfont}

% more options: leftmargin=*, topsep=2pt, partopsep=0pt, labelindent=3pt
\setitemize{itemsep=0pt, parsep=0pt} 				% adjust itemize environment
\setenumerate{itemsep=0pt, parsep=0pt} 				% adjust enumerate environment
\renewcommand{\thefootnote}{\fnsymbol{footnote}} 	% footnote symbol
\setlength{\tabcolsep}{5pt}		% adding space between columns in a table
%\setlength{\parskip}{5pt} 		% parameter that characterises the paragraph spacing
%\setlength{\parindent}{0pt} 	% parameter that characterises the paragraph indentation

% maximal number of floating environments on each page (default values)
%\setlength{\floatsep}{0pt} 			% vertical space between floating objects
%\setcounter{topnumber}{2} 				% maximum number of floats at top of page 
%\setcounter{bottomnumber}{1} 			% maximum number of floats at bottom of page 
%\setcounter{totalnumber}{3} 			% maximum number of floats on a page
%\renewcommand{\topfraction}{0.7} 		% maximum fraction of page for floats at top
%\renewcommand{\bottomfraction}{0.3} 	% maximum fraction of page for floats at bottom
%\renewcommand{\textfraction}{0.2} 		% minimum fraction of page for text

% To fix list things: 
\setitemize{itemsep=2pt,topsep=2pt,parsep=0pt,partopsep=0pt,leftmargin=*}
\setenumerate{itemsep=0pt,topsep=2pt,parsep=0pt,partopsep=0pt,labelindent=3pt,leftmargin=*}
\setlength{\tabcolsep}{2pt}


